A framework for optimisation based stochastic process discovery

Process mining is concerned with deriving formal models capable of reproducing the behaviour of a given organisational process by analysing observed executions collected in an event log. The elements of an event log are finite sequences (i.e., traces or words) of actions. Many effective algorithms have been introduced which issue a control flow model (commonly in Petri net form) aimed at reproducing, as precisely as possible, the language of the considered event log. However, given that identical executions can be observed several times, traces of an event log are associated with a frequency and, hence, an event log inherently yields also a stochastic language. By exploiting the trace frequencies contained in the event log, the stochastic extension of process mining, therefore, consists in deriving stochastic (Petri nets) models capable of reproducing the likelihood of the observed executions. In this paper, we introduce a novel stochastic process mining approach. Starting from a "standard" Petri net model mined through classical mining algorithms, we employ optimization to identify optimal weights for the transitions of the mined net so that the stochastic language issued by the stochastic interpretation of the mined net closely resembles that of the event log. The optimization is either based on the maximum likelihood principle or on the earth moving distance. Experiments on some popular real system logs show an improved accuracy w.r.t. to alternative approaches.

==> pic_latex/table2.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l p{1ex} c c p{1ex} c c p{1ex} c c}
        \toprule 
        Event log & & \multicolumn{2}{l}{log properties} & & \multicolumn{2}{l}{net properties} & & \multicolumn{2}{l}{reachability graph}\\
        \cmidrule(){3-4} \cmidrule(){6-7} \cmidrule(){9-10}
         & & \#dpi & \#at & & \#pl & \#tr & & \#state & \#tr \\
        \hline
        BPIC13\_c & & 183 & 4 & & 16 & 19 & & 46 & 176 \\
        BPIC13\_i & & 1511 & 4 & & 17 & 23 & & 90 & 352 \\
        BPIC13\_o & & 108 & 3 & & 16 & 20 & & 74 & 264 \\ 
        BPIC17\_ol & & 16 & 8 & & 6 & 11 & & 6 & 11 \\
        BPIC20\_dd & & 99 & 17 & & 26 & 43 & & 235 & 1147 \\
        BPIC20\_rfp & & 89 & 19 & & 33 & 51 & & 247 & 1292 \\
        Roadfines & & 231 & 11 & & 29 & 34 & & 906 & 6526 \\
        \bottomrule
    \end{tabular}
    \caption{Event logs, nets and reachability graphs statistics.}
    \label{tab:prop}
\end{table}


==> pic_latex/table3.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l p{1ex} l l l p{2ex} c l p{2ex} c l}
        \toprule 
        Event log & & \multicolumn{3}{l}{Computation time} & & \multicolumn{2}{l}{LH-opt} & & \multicolumn{2}{l}{rEMD-opt} \\
        \cmidrule(){3-5} \cmidrule(){7-8} \cmidrule(){10-11}
         & & unfold & LH & rEMD & & $\sharp$iter & time & & $\sharp$iter & time \\
        \hline
        BPIC13\_c & & 0.18 & 0.00029 & 0.096 & & 4 & 36.58 & & 8 & 603.12 \\
        BPIC13\_i & & 8.15 & 0.0046 & 8.06 & & 4 & 1913.23 & & 8 & 87086.48 \\
        BPIC13\_o & & 0.072 & 0.00025 & 0.036 & & 8 & 35.18 & & 6 & 137.68 \\
        BPIC17\_ol & & 0.00029 & 2.05e-05 & 0.00057 & & 12 & 0.11 & & 11 & 1.27 \\
        BPIC20\_dd & & 0.19 & 0.00027 & 0.035 & & 14 & 296.32 & & 31 & 3946.85 \\
        BPIC20\_rfp & & 0.48 & 0.0003 & 0.025 & & 7 & 572.85 & & 11 & 59819.73 \\
        Roadfines & & 1.01 & 0.0014 & 0.16 & & 5 & 204.3 & & 4 & 1276.95 \\
        \bottomrule
    \end{tabular}
    \caption{Computation time  (in seconds) for weight optimisation.}
    \label{tab:time}
\end{table}


==> sections/1_intro_pierre.tex <==
Understanding business processes is a primary goal for organizations to get significant insights and optimize their operations. Today's real-life process information system dispenses a large number of data that needs to be synthesized to get readable and computable models. Those data take the form of a list of activities performed by identified entities at a known time and day, called an event log. Process discovery aims to discover a meaningful process model that reflects behaviors observed in a log. Petri nets are widely used as a model formalism thanks to their expressiveness in translating workflows. For a few years, process discovery has enlightened a lot about establishing a causal relationship between log activities for the purpose of construing those precedence and successor relations inside the goal model. However, this control flow aspect only deprives the model of a set of features stored in the log, such as stochastic characteristics. It is usually essential for a model to translate the likelihood of one event over another. For instance, after a particular series of medical check-ups in a hospital, it is helpful to know the most likely next one to be carried out to optimize the hospital resources around this particular department.

Stochastic process mining is interested in deriving stochastic models capable of reproducing the likelihood of executions observed on an event log. In the language over the alphabet of activities deriving from an event log, each unique sequence (i.e. trace) has a frequency attached that gives the number of times each one of them appeared in the log. Consequently, an event log yields a stochastic language, a language whose words are given by the traces contained in the event log and whose probability is given by the proportion of a trace w.r.t. to the total number of collected executions. More specifically, the aim of stochastic process mining is to derive a probabilistic model whose corresponding stochastic language is as close as possible to the event log's. The stochastic aspect can be modeled by a stochastic extension of the Petri net definition and controlled by a function that assigns positive real weights to the net component.

==> sections/2_preliminaries_pierre.tex <==
\section{Preliminaries - Pierre}

A \textit{language} is a multiset of sequence over an alphabet $\Sigma$. For instance, $[\langle a, b, d \rangle^{2}, \langle a, c \rangle]$ is the language containing the same sequence $\langle a, b, d \rangle$ two times and the unique sequence $\langle a, c \rangle$ over an alphabet $\Sigma = \{a, b, c, d\}$.

A \textit{Stochastic language} is a set of sequences over an alphabet $\Sigma$ with attached probabilities. Formally, a stochastic language is a function $f : \Sigma^{*} \rightarrow [0,1]$ that map each word onto a probability such that $\sum_{w \in \Sigma^*}f(t) = 1$. For instance, $[\langle a, b, d \rangle^{\frac{2}{3}}, \langle a, c \rangle^{\frac{1}{3}}]$ is a stochastic language with two sequences, the first one has a probability of $\frac{2}{3}$.

An \textit{event log} $L$ is a collection of events. Each event contains multiple features, but three of them are mandatory: a unique case that identifies the entity performing the event, an activity, and a timestamp that gives us what happened and when it occurred. By looking at every time-ordering sequence of activity, called trace, performed by each case, we can build the event log language $\mathcal{L}(L)$, which is the multiset of trace over the alphabet of activity $\Sigma$. From the language, we can extract the event log stochastic language $\mathcal{L}_s(L)$ by normalizing the trace quantities by dividing each trace's occurrence in the multiset by the total number of traces, giving the probability of each trace in the log.

A \textit{labeled Petri net} is a tuple $N = \langle P, T, F, m_0, \Sigma, \lambda \rangle$, where $P$ is a finite set of places, $T$ is a finite set of transitions such that $P \cap T = \emptyset$, $F : (P \times T) \rightarrow (T \times P)$ is the flow relation, $\Sigma$ is a finite alphabet of activity and $\lambda: T \rightarrow \Sigma \cup \{\tau\}$ is a labeling function such as $\tau \notin \Sigma$. A marking is a multiset of places $\in P$, indicating the number of tokens in each place, which describes the net state. $m_0$ is the initial marking. A transition is enabled if every incoming place contains at least a token. Firing a transition changes the marking of the net by consuming a token in each incoming place of the transition and producing a token in each outcoming edge of the transition. If a transition $t \in T$ is labeled by an activity $\lambda(t) \in \Sigma$, then firing $t$ corresponds to the execution of the discrete event $\lambda(t)$. Suppose a transition $t$ is labeled by the silent activity $\tau$; the firing $t$ changes the state of the net without executing an event. A path through the model is a sequence of transition firings, starting from the initial marking and ending in a state without enabled transitions, called a deadlock. The corresponding label of each transition in the path allows us to create a trace from the alphabet $\Sigma$. The possibly non-finite set of trace derived from the possibly non-finite set of paths in the net gives us the language of the labeled Petri net $N$, written $\mathcal{L}(N)$.

A \textit{labeled workflow net} is a \textit{labeled Petri net} $N = \langle P, T, F, m_0, \Sigma, \lambda \rangle$ fulfilling multiple structural properties:
\begin{itemize}
    \item P contains a unique place, called the start place, without incoming transition and another unique place, called the end place, without outcoming transition,
    \item $m_0 = [start]$,
    \item every flow multiplicity is equal to 1 and
    \item a Petri net $\bar{N} = (P,\bar{T},\bar{F},m_0,\Sigma,\lambda)$ can be built by adding a transition $\bar{t}$ in $N$ connecting the end and the start place $(\bar{T} = T \cup \{\bar{t}\}$ and $\bar{F} = F \cup \{(o,\bar{t}),(\bar{t},i)\})$ making $\bar{N}$ strongly connected.
\end{itemize}

A \textit{generalized stochastic labeled Petri net (GSLPN)} is a tuple $G = \langle P, T, F, m_0, \Sigma, \lambda, W, T_i, T_t \rangle$ where $\langle P, T, F, m_0, \Sigma, \lambda \rangle$ is a labeled Petri net. $T_i \subseteq T$ is the set of immediate transition and $T_t \subseteq T$ is the set of timed transition such as $T_i \cap T_t = \emptyset$. $W : T \rightarrow \mathbb{R}^{+}$ is the function assigning a weight to each transition. Timed transition cannot fire when at least one immediate transition is enabled. If multiple immediate transitions $T_i^{'} \subseteq T_i$ are enabled in the same marking, the probability of firing a transition $t \in T_i^{'}$ is $\frac{W(t)}{\sum_{t^{'} \in T_i^{'}} W(t^{'})}$. A timed transition follows an exponentially distributed law with a firing rate parameter $W(t)$. Due to exponential distribution properties, when multiple timed transition $T_t^{'} \subseteq T_t$ are enabled in the same marking, the transition $t$ fire first with the probability $\frac{W(t)}{\sum_{t^{'} \in T_i^{'}} W(t^{'})}$. The probability of a transition is marking dependent. The probability of a trace is given by the sum of the probabilities over all paths through the model that produces the trace following the labels assigned given by $\lambda$. Given a certain path, its probability is the product of the probabilities of firing each path transition. The possibly non-finite set of traces with attached probabilities derived from the possibly non-finite set of paths gives us the stochastic language of the GSLPN $\mathcal{L}_s(G)$.

For instance, Figure 1 shows a GSLPN with four places and six immediate transitions labeled over the alphabet $\{a, b, c, d\}$. Transition $t_1$ is labeled with the silent activity $\tau$ and $t_2$ and $t_3$ are labeled with the same activity $b$. There is 3 possible path leading from the initial marking $m_0 = [start]$ to the only deadlock marking $m_f = [end]$ resulting into the following 2 traces:
\begin{itemize}
    \item For $\langle a,b,d \rangle$ : 
        \[ P(\langle t_0, t_1, t_2, t_5 \rangle) + P(\langle t_0, t_3, t_5 \rangle) = (P(t_0)*P(t_1)*P(t_2)*P(t_5)) + (P(t_0)*P(t_3)*P(t_5)) = \frac{1}{3} + \frac{1}{2} = \frac{10}{12} \]
    \item For $\langle a,c \rangle$ : 
        \[ P(\langle t_0, t_4 \rangle) = P(t_0) * P(t_4) = \frac{1}{6} \]
\end{itemize}

==> sections/6_garbage.tex <==
\section{Garbage collector}
\begin{algorithm}
\caption{Reachability graph unfolding to compute trace probabilities\label{alg:unfold}}
\begin{algorithmic}[1]
  \Function{UnfoldRG}{Reachability Graph $R$, Traces $T$}
  \State $Q \leftarrow$ empty queue
  \State $Q$.\Call{Enqueue}{$<initial~state~of~R, 0, empty~trace>$
    associated with prob. 1}
  \State $D\leftarrow$ empty dictionary
  \While{$Q$ is not empty}
  \State $<st, level, tr>~\leftarrow$ $Q$.\Call{Dequeue}{$~\!$} \label{alg:dequeue}
  \State $pr \leftarrow$ probability associated with $<st, level, tr>$
  \For{$\forall$ outgoing arc $a$ of $st$} \label{alg:outg}
  \State $newst~\leftarrow~a.tostate$ \label{alg:newst}
  \State $newtr~\leftarrow~t+a.label$
  \State $newpr~\leftarrow pr \cdot a.prob$ \label{alg:newprob}
  \If{$newst$ is the sink} \label{alg:sink}
  \If{$newtr$ is a trace in $T$}
  \State $D$.\Call{AddOrIncrease}{$newtr$, $newpr$}
  \EndIf \label{alg:endsink}
  \ElsIf{$newtr$ is prefix of a trace in $T$}
  \State $Q$.\Call{AddOrIncrease}{$<newst,level+1,newtr>$, $newpr$}
  \EndIf
  \EndFor
  \EndWhile
  \State\Return{$D$}
  \EndFunction
\end{algorithmic}
\label{alg:slg}
\end{algorithm}


